Fast, Accurate, and Scalable Method for Sparse Coupled Matrix-Tensor Factorization

How can we capture the hidden properties from a tensor and a matrix data simultaneously in a fast, accurate, and scalable way? Coupled matrix-tensor factorization (CMTF) is a major tool to extract latent factors from a tensor and matrices at once. Designing an accurate and efficient CMTF method has become more crucial as the size and dimension of real-world data are growing explosively. However, existing methods for CMTF suffer from lack of accuracy, slow running time, and limited scalability. In this paper, we propose S3CMTF, a fast, accurate, and scalable CMTF method. S3CMTF achieves high speed by exploiting the sparsity of real-world tensors, and high accuracy by capturing inter-relations between factors. Also, S3CMTF accomplishes additional speed-up by lock-free parallel SGD update for multi-core shared memory systems. We present two methods, S3CMTF-naive and S3CMTF-opt. S3CMTF-naive is a basic version of S3CMTF, and S3CMTF-opt improves its speed by exploiting intermediate data. We theoretically and empirically show that S3CMTF is the fastest, outperforming existing methods. Experimental results show that S3CMTF is 11~43 times faster, and 2.1~4.1 times more accurate than existing methods. S3CMTF shows linear scalability on the number of data entries and the number of cores. In addition, we apply S3CMTF to Yelp recommendation tensor data coupled with 3 additional matrices to discover interesting properties.

==> 050related.tex <==
In this section, we review related works on coupled matrix-tensor factorization.

\subsection{Coupled Matrix-Tensor Factorization}
To analyze tensor data with additional information matrices, Acar et al. \cite{acar2011all} present CMTF-OPT, a gradient descent, single machine CMTF algorithm 

There are some ways to make a proximity matrix to couple to a mode of a tensor. \cite{ozcaglar2012host} suggests to formulate the proximity matrix as the cosine distance between features between entries.
